Structural Results for Partially Observed Markov Decision Processes

This article provides an introductory tutorial on structural results in partially observed Markov decision processes (POMDPs). Typically, computing the optimal policy of a POMDP is computationally intractable. We use lattice program- ming methods to characterize the structure of the optimal policy of a POMDP without brute force computations.

==> part0/figures/sensadapt.tex <==
%!TEX root = ../book.tex

\begin{pspicture}[showgrid=false](0.5,-0.5)(14,2.1)

%--- Define blocks ---


\dotnode[dotstyle=square*,dotscale=0.001](12.5,0.75){dot}



\psblock(2,.75){H1}{\begin{tabular}{c} Stochastic \\ Dynamical \\ System \end{tabular}}

\psblock(6,.75){B2}{\begin{tabular}{c} Noisy \\ Sensor \end{tabular}}

\psblock(10,.75){B1}{\begin{tabular}{c} Signal \\ Processing  \\ Algorithm \end{tabular}}

%\pscircleop(7.7,0){ominus}

%\rput(9,0){\rnode{e}{$e[n]$}}

 

%--- Connect blocks ---

\psset{style=Arrow}


\ncline{H1}{B2} \naput[npos=.5]{State}
\nbput[npos=.5]{$\state_k$}

\ncline{B2}{B1} \nbput[npos=.5]{$\obs_k$}
\naput[npos=.5]{Observation}

\ncline{B1}{dot} \naput[npos=.5]{Estimate}



\end{pspicture}


==> part0/figures/sensadapt2.tex <==
\begin{pspicture}[showgrid=false](0.5,-2)(14,2.55)

%--- Define blocks ---


\dotnode[dotstyle=square*,dotscale=0.001](12.5,0.75){dot}



\psblock(2,.75){H1}{\begin{tabular}{c} Stochastic \\ Dynamical \\ System \end{tabular}}

\psblock(6,.75){B2}{\begin{tabular}{c} Noisy \\ Sensor \end{tabular}}

\psblock(10,.75){B1}{\begin{tabular}{c} Signal \\ Processing  \\ Algorithm \end{tabular}}

\psblock(9,-1.75){B3}{\begin{tabular}{c} Stochastic\\ Controller \end{tabular}}

%\pscircleop(7.7,0){ominus}

%\rput(9,0){\rnode{e}{$e[n]$}}

 

%--- Connect blocks ---

\psset{style=Arrow}


\ncline{H1}{B2} \naput[npos=.5]{State}
\nbput[npos=.5]{$\state_k$}

\ncline{B2}{B1} \nbput[npos=.5]{$\obs_k$}
\naput[npos=.5]{Observation}

\ncline{B1}{dot} \naput[npos=.5]{Estimate}

\ncangle[angleA=0,angleB=180]{B3}{dot}

\ncangle[angleA=180,angleB=-90]{B3}{B2}
 \nbput[npos=.5]{Action}
 \naput[npos=.5]{$\action_k$}

\end{pspicture}


==> part0/figures/stateobs.tex <==
%!TEX root = ../book.tex

\begin{pspicture}[showgrid=false](0.5,0)(12,2.55)

%--- Define blocks ---


\dotnode[dotstyle=square*,dotscale=0.001](10,0.75){dot}



\psblock(2,.75){H1}{\begin{tabular}{c} Stochastic \\ Dynamic \\ System \end{tabular}}

\psblock(6,.75){B2}{\begin{tabular}{c} Noisy \\ Sensor \end{tabular}}

%\psblock(12,.75){B1}{\begin{tabular}{c} Signal \\ Processing  \\ Algorithm \end{tabular}}

%\pscircleop(7.7,0){ominus}

%\rput(9,0){\rnode{e}{$e[n]$}}

 

%--- Connect blocks ---

\psset{style=Arrow}


\ncline{H1}{B2} \naput[npos=.5]{state}
\nbput[npos=.5]{$\state_k$}

\ncline{B2}{dot} \nbput[npos=.5]{$\obs_k$}
\naput[npos=.5]{observation}

%\ncline{B1}{dot} \naput[npos=.5]{Estimate}



\end{pspicture}


==> part2/figures/mdpfig.tex <==
\begin{pspicture}[showgrid=false](0.5,-1.5)(8,1.55)
\psblock(4,1){H1}{\begin{tabular}{c} Markovian \\ System \end{tabular}}
\psblock(4,-.75){H2}{\begin{tabular}{c} Controller \\ Lookup Table \end{tabular}}
\ncangle[angleA=0,angleB=0,arrows=->]{H1}{H2}\naput[npos=.75]{$\state_k$}
\ncangle[angleA=180,angleB=180,armB=1cm,arrows=->]{H2}{H1}\naput[npos=0.75]{$\action_k$}
\end{pspicture}
